EdgeSight: Enabling Modeless and Cost-Efficient Inference at the Edge

Traditional ML inference is evolving toward modeless inference, which abstracts the complexity of model selection from users, allowing the system to automatically choose the most appropriate model for each request based on accuracy and resource requirements. While prior studies have focused on modeless inference within data centers, this paper tackles the pressing need for cost-efficient modeless inference at the edge -- particularly within its unique constraints of limited device memory, volatile network conditions, and restricted power consumption. To overcome these challenges, we propose EdgeSight, a system that provides cost-efficient EdgeSight serving for diverse DNNs at the edge. EdgeSight employs an edge-data center (edge-DC) architecture, utilizing confidence scaling to reduce the number of model options while meeting diverse accuracy requirements. Additionally, it supports lossy inference in volatile network environments. Our experimental results show that EdgeSight outperforms existing systems by up to 1.6x in P99 latency for modeless services. Furthermore, our FPGA prototype demonstrates similar performance at certain accuracy levels, with a power consumption reduction of up to 3.34x.

==> texts/acknowledgement.tex <==
\section*{Acknowledgments}
Acknowledgements

==> texts/design.tex <==
\section{Design}\label{sec:design} 

% \subsection{Overview}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/system_overview.png}
% 	\caption{Redraw later - System Overview}
%     \label{fig:system_overview}
% \end{figure}


% \sysname system (Figure~\ref{fig:system_overview}) target is to provide low latency, high throughput prediction service while handling uncertain network issues with negligible accuracy compromise. 

% The {\bf client} module first takes input JPEG images from the user, through \sysname's API and send it to the target prediction system every when user make an inference request. The requests afterwards go both {\bf End-host slow path} and {\bf NIC fast path} for the inference from the SmartNIC. The fast path reply answer directly when the answer is credible, while the slow path act as original CPU+GPU workflow.

% \subsection{Client}
% \label{sec:client} 
% Before every request, the client proxy extracts the JPEG block locations in the first stage. These information help NIC to recover of the image and identify the packet loss without CPU participate. The JPEG knowledge will be encoded to the \sysname packets and send with the JPEG stream.


% \subsubsection{JPEG Knowledge Parsing}
% \label{sec:jpeg_parsing} 
% The client parse the locations of Minimum Coded Units (MCUs) from the JPEG image in the first place. We modified libjpeg-turbo~\cite{libjpeg-turbo} for this purpose. The cost analysis can be found in Appendix~\cite{}.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/packet_format.png}
% 	\caption{Redraw later - \sysname packet format}
%     \label{fig:packet_format}
% \end{figure}

% \subsubsection{Communication Module}
% \label{sec:client_communication}
% After acquiring the MCU locations, the communication module construct the packets as Figure~\ref{fig:packet_format}. Each packet contains \codesm{MCU\_Start} and \codesm{MCU\_End}, which are obtained from the JPEG parsing stage (\secref{sec:jpeg_parsing}), along with the JPEG streaming data.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/nic_overflow.png}
% 	\caption{Redraw later - NIC Overview \lam{add output format for the figure, poss+ans}}
%     \label{fig:nic_overview}
% \end{figure}

% \subsection{NIC - the Fast Path}
% Figure~\ref{fig:nic_overview} shows the FPGA NIC design. There are five main components in the FPGA in a streaming manner: {\bf(1) Packet Parser}: the parser is the entrance point of the \sysname inference flow, filtering out all the non-\sysname-related packets with specific header field. This component is written in P4 language~\cite{p4}. \lam{don't know if we can mentioned VitisP4Net publicly, I'll ask Gorden}. {\bf(2) JPEG reformer}: the reformer detects the packet loss and recover the JPEG image when loss happened. This component stores the last seen MCU status for every incoming packets and keep track on the discontinuous MCUs. When discontinuous happens (e.g., the last seen MCU != \codesm{MCU\_Start} of the incoming packet), the reformer inserts the missing MCUs by duplicating the first MCU of the incoming packet multiple times. The justification of this design can be found in Section~\ref{}. After the reformer, the \sysname header will be striped off and flows the pure JPEG data stream to the next component. {\bf(3) JPEG decoder}: the JPEG decoder receives the JPEG stream data from the previous component. Our design does not include the modification of the JPEG decoder. Since recovered the JPEG stream in the previous component, the stall of the decoding process due to the missing piece of data stream is avoided. {\bf(4) Image Preprocessing}: before feeding into the image classification inference model, we need to preprocess the image data as endhost's CPU do. We implemented resize and crop functions in this component in Vitis HLS vision Library~\cite{vitis_vision}. All the images are cropped into the specific input format of the inference model. {\bf(5) Model Inference}: the processed image eventually flows into the classification model. Our design uses MobileNet complied by Xilinx FINN~\cite{blott2018finn, finn} as a demonstration. Any FPGA image classification models~\cite{DBLP:conf/icfpt/PetricaAKFCB20,DBLP:journals/corr/abs-2007-10451,10.1145/3404397.3404473,10.1145/3289602.3293915,8825027,10.1145/3330345.3330385,8416814,DBLP:journals/corr/abs-1806-01683,10.1145/3289185,10.1145/3174243.3174266} can be fit into this component. The output of this component are prediction answer with corresponding possibility. We identify the output possibilities of a model as confidence score, representing if the answer is "trustable" as long as the model is well-calibrated~\cite{pmlr-v70-guo17a, Vemuri:EECS-2020-132, NEURIPS2021_8420d359}. This is evaluated in Section~\ref{}. {\bf(6) Result arbiter}: when the NIC finish an request, it has two ways to go as Figure~\ref{fig:nic_overview} shown. If the confidence score exceed a certain threshold, the NIC reply the trustable answer directly to the client and notify the end-host for the completion. This cause the removal of the queuing request and release the GPU computation resource.


% \subsection{Endhost - the Slow Path}
% Our end-host inference server handles all the \sysname traffic sent by the client proxy, along with the notification packets generated by the SmartNIC. After reassembled the packets, the system is identical to any inference workflow. For the end-host, FPGA NIC is invisible and has the same role of commodity NICs.

% \subsection{Best Effort}
% \subsubsection{Confidence Score}
% We use model output possibility to determine the confidence of the answer given~\cite{pmlr-v70-guo17a, Vemuri:EECS-2020-132, NEURIPS2021_8420d359}. The confidence score is to decide if the answer should return to the user from the NIC directly, or fall back to the end-host large model for a more confidence result. Our modified FINN~\cite{blott2018finn, finn} gives the answer with corresponding possibility for each inference. Once the inference answer and possibility is generated, it compare to the confidence threshold: (1) if the confidence score is large then the threshold: the NIC send back the result with a answer packet, and notify the end-host that the inference is already handled by the NIC. (2) if the confidence score is smaller then the threshold: the NIC will ignore the answer and wait for end-host to finish the results as usual. 

% \subsection{Why and is Confident Score work?}

% Figures \ref{fig:boundary_fpga},~\ref{fig:boundary_gpu}.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\linewidth]{figures/designs/threshold_analysis/confident_score_useful_FPGA.png}
% 	\caption{The boundary of true/false prediction is clear (GPU) \lam{move to motivation?}}
%     \label{fig:boundary_fpga}
% \end{figure}


% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\linewidth]{figures/designs/threshold_analysis/confident_score_useful_GPU.png}
% 	\caption{The boundary of true/false prediction is clear (GPU) \lam{move to motivation?}}
%     \label{fig:boundary_gpu}
% \end{figure}

% \subsubsection{Packet Loss}
% The NIC handled the packet loss without the need of resent packets. Our results (Section \ref{}) demonstrate that the miss of partial information within an image does not cause significant accuracy drop in inference. When packet loss happen (the NIC receive discontinuous sequence number), our JPEG reformer (Section \ref{}) duplicates the JPEG blocks and insert into the JPEG decoding stream. 

% In this design, we make a trade-off between waiting for the resend packets and the drop of the accuracy since the role of our NIC is to perform low-latency and best effort inference. Further, we leave the packet loss handling protocol to the end-host for the full image. When the NIC results made by partial information input is not confidence enough (\ref{}), the end-host will always finished the request with full information of the images even though it will be slower due to the retransmission handling.

% \subsection{Why and is partial JPEG image work?}
% \lam{How missing JPEG do not affect the accuracy}
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\linewidth]{figures/designs/partial_image/partial_image_accuracy.png}
% 	\caption{Partial Image v.s. Accuracy \lam{move to motivation?}}
%     \label{fig:partial_image_accuracy}
% \end{figure}
